Quantifier Instantiations: To Mimic or To Revolt?

Quantified formulas pose a significant challenge for Satisfiability Modulo Theories (SMT) solvers due to their inherent undecidability. Existing instantiation techniques, such as e-matching, syntax-guided, model-based, conflict-based, and enumerative methods, often complement each other. This paper introduces a novel instantiation approach that dynamically learns from these techniques during solving. By treating observed instantiations as samples from a latent language, we use probabilistic context-free grammars to generate new, similar terms. Our method not only mimics successful past instantiations but also explores diversity by optionally inverting learned term probabilities, aiming to balance exploitation and exploration in quantifier reasoning.

==> picture.tex <==
% File: picture.tex
% Author: mikolas
% Created on: Fri May 9 09:52:22 CEST 2025
% Copyright (C) 2025, Mikolas Janota

\begin{tikzpicture}[
    box/.style={draw, thick, minimum width=2.5cm, minimum height=1em, align=center},
    circle node/.style={draw, circle, fill=white, inner sep=2pt},
    arrow/.style={->, >=Stealth, thick},
    node distance=2em,
    yscale=.4
]

% \node[align=center, font=\Large\bfseries] at (0,5) {Instantiation modules};

% Boxes
\node[box,fill=green!20] (module1) at (-3,0.5) {Inst.\ module 1};
\node[box,fill=green!20] (module2) at (-3,-1) {Inst.\ module 2};
\node (dots) at (-3,-2.5) {$\ldots$};
\node[box, align=center,fill=red!20] (probgen) at (0,-5) {\textsc{Probgen}};
\node[box, align=center,fill=green!20] (solver) at (3,0.5) {Ground Solver};

% Connection points
\node[circle node] (c1) at (0,.5) {};
\draw[arrow] (c1) -- (probgen);
\node[circle node] (c2) at (0,-1) {};
\node[circle node] (c3) at (0,-2.5) {};

% Arrows
\draw[arrow] (module1) -- (c1);
\draw[arrow] (module2) -- (c2);
\draw[arrow] (dots) -- (c3);
\draw[arrow] (c1) -- (solver);
\draw[arrow] (c2) -| (solver.south west);
\draw[arrow] (c3) -| (solver);
\draw[arrow] (probgen) -| (solver.south east);
% \draw[arrow] (solver) |- (probgen);

\end{tikzpicture}

